Demotivate adversarial defense in remote sensing

Convolutional neural networks are currently the state-of-the-art algorithms for many remote sensing applications such as semantic segmentation or object detection. However, these algorithms are extremely sensitive to over-fitting, domain change and adversarial examples specifically designed to fool them. While adversarial attacks are not a threat in most remote sensing applications, one could wonder if strengthening networks to adversarial attacks could also increase their resilience to over-fitting and their ability to deal with the inherent variety of worldwide data. In this work, we study both adversarial retraining and adversarial regularization as adversarial defenses to this purpose. However, we show through several experiments on public remote sensing datasets that adversarial robustness seems uncorrelated to geographic and over-fitting robustness.

==> old_tables.tex <==
%%%%%table 1
% initial
\begin{table}
\begin{center}
\begin{tabular}{c||c|c|c|c}
\multirow{2}{*}{\diagbox[]{Training}{Testing}} & AIRS  & ISPRS  & AIRS & ISPRS\\
 & \textit{clean} & \textit{clean} & \textit{adv} & \textit{adv}
\\\hline\hline
AIRS & 94 & 75 & 88 & 61\\\hline
AIRS + extra data & \textbf{98} & \textbf{91} & 87 & \textbf{83} \\\hline
AIRS + \textit{adv} & 92 & 78 & \textbf{91} & 74 \\

\end{tabular}

\caption{\label{segmentation} Root segmentation accuracy depending on train/test data.
Test data can be with (\textit{adv}) or without (\textit{clean}) adversarial attacks and training can be \textit{naive}, with adversarial defence (\textit{adv}) or with extra data (INRIA + DFC).}
\end{center}
\end{table}

%with booktabs
\begin{table}
\begin{center}
\begin{tabular}{c|cccc}
\toprule
\multirow{2}{*}{\diagbox[]{Train}{Test}} & AIRS  & ISPRS  & AIRS & ISPRS\\
 & \textit{clean} & \textit{clean} & \textit{adv} & \textit{adv}
\\
\midrule
AIRS & 94 & 75 & 88 & 61\\
AIRS + \textit{add} & \textbf{98} & \textbf{91} & 87 & \textbf{83} \\
AIRS + \textit{adv} & 92 & 78 & \textbf{91} & 74 \\
\bottomrule
\end{tabular}
\caption{\label{segmentation} Root segmentation accuracy depending on train/test data.
Test data can be with (\textit{adv}) or without (\textit{clean}) adversarial attacks and training can be \textit{naive}, with adversarial defence (\textit{adv}) or with extra data (INRIA + DFC) \textit{(add)}.}
\end{center}
\end{table}



%%%%%table 2
%original
\begin{table*}[h!]
\begin{center}

\begin{tabular}{c||c|c|c || c | c |c }
\multirow{2}{*}{\diagbox[]{Model}{Dataset}} & VEDAI  & DFC  & ISPRS & VEDAI & DFC & ISPRS\\
 & \textit{32$\times$32} & \textit{48$\times$48} & \textit{64$\times$64} & \textit{adv} & \textit{adv} & \textit{adv}
\\\hline\hline
VGG & 53 & 66 & 78 & 30 & 51 & 66\\\hline
VGG reg & 53 & 65 & 80 & \textbf{36} & \textbf{57} & \textbf{74}\\\hline
VGG add & \textbf{62} & \textbf{71} & \textbf{85} &31 & 49 & 64\\\hline\hline
RESNET & 39 & 60 & 80 & 22 & 24 & 50\\\hline
RESNET reg & 43 & 49 & 81 & 20 & \textbf{29} & \textbf{69}\\\hline
RESNET add & \textbf{57} & \textbf{65} & \textbf{82} & 21 & 26 & 52

\end{tabular}
\caption{\label{detection} G score performances of naive detector, adversarial defended detector (\textit{reg}) and detector with extra data (\textit{add}) on clean and adversarial (\textit{adv}) VEDAI, DFC and ISPRS. \textit{Target size in different dataset is indicated in italic for completeness.}}
\end{center}
\end{table*}













%%%%%%%%%%%%%%%%%%%%%%%% Both tables before minipage

\begin{table}
\begin{center}
\begin{tabular}{c|ccc}
\toprule
\multirow{2}{*}{\diagbox[]{Test}{Train}} & AIRS  & AIRS  & AIRS\\
 & \textit{naive} & \textit{add} & \textit{adv} \\
\midrule
AIRS \textit{clean} & 94 & \textbf{98} & 92\\
ISPRS \textit{clean} & 75 & \textbf{91} & 78 \\
AIRS \textit{adv} & 88 & 87 & \textbf{91}\\
ISPRS \textit{adv} & 61 & \textbf{83} & 74 \\
\bottomrule
\end{tabular}
\caption{\label{segmentation} Root segmentation accuracy depending on train/test data.
Test data can be with (\textit{adv}) or without (\textit{clean}) adversarial attacks and training can be \textit{naive}, with adversarial defence (\textit{adv}) or with extra data (INRIA + DFC) \textit{(add)}.}
\end{center}
\end{table}





\begin{table*}[h!]
\begin{center}

\begin{tabular}{c|ccc || c  c c }
\toprule
\multirow{2}{*}{\diagbox[]{Model}{Dataset}} & VEDAI  & DFC  & ISPRS & VEDAI & DFC & ISPRS\\
 & \textit{32$\times$32} & \textit{48$\times$48} & \textit{64$\times$64} & \textit{adv} & \textit{adv} & \textit{adv}

\\ \midrule
VGG & 53 & 66 & 78 & 30 & 51 & 66\\
VGG reg & 53 & 65 & 80 & \textbf{36} & \textbf{57} & \textbf{74}\\
VGG add & \textbf{62} & \textbf{71} & \textbf{85} &31 & 49 & 64\\\hline\hline
RESNET & 39 & 60 & 80 & 22 & 24 & 50\\
RESNET reg & 43 & 49 & 81 & 20 & \textbf{29} & \textbf{69}\\
RESNET add & \textbf{57} & \textbf{65} & \textbf{82} & 21 & 26 & 52\\
\bottomrule
\end{tabular}

\caption{\label{detection} G score performances of naive detector, adversarial defended detector (\textit{reg}) and detector with extra data (\textit{add}) on clean and adversarial (\textit{adv}) VEDAI, DFC and ISPRS. \textit{Target size in different dataset is indicated in italic for completeness.}}
\end{center}
\end{table*}
